Report of the Topical Group on Wave Dark Matter for Snowmass 2021

There is a strong possibility that the particles making up the dark matter in the Universe have a mass below 1 eV and in many important situations exhibit a wave-like behavior. Amongst the candidates the axion stands out as particularly well motivated but other possibilities such as axion-like particles, light scalars and light vectors, should be seriously investigated with both experiments and theory. Discovery of any of these dark matter particles would be revolutionary. The wave-like nature opens special opportunities to gain precise information on the particle properties a well as astrophysical information on dark matter shortly after a first detection. To achieve these goals requires continued strong support for the next generations of axion experiments to probe significant axion parameter space this decade and to realize the vision of a definitive axion search program in the next 20 years. This needs to be complemented by strong and flexible support for a broad range of smaller experiments, sensitive to the full variety of wave-like dark matter candidates. These have their own discovery potential but can also be the test bed for future larger scale searches. Strong technological support not only allows for the optimal realization of the current and near future experiments but new technologies such as quantum measurement and control can also provide the next evolutionary jump enabling a broader and deeper sensitivity. Finally, a theory effort ranging from fundamental model building over investigating phenomenological constraints to the conception of new experimental techniques is a cornerstone of the current rapid developments in the search for wave-like dark matter and should be strengthened to have a solid foundation for the future.

==> CF2_authors.tex <==
%\author[7]{\\ \textbf{Contributors:} Daniel S. Akerib}

%\affil[7]{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

